Measurement of ZZ production in pp collisions at sqrt(s)=7 TeV and limits on anomalous ZZZ and ZZgamma couplings with the ATLAS detector

A measurement of the ZZ production cross section in proton-proton collisions at sqrt(s) = 7 TeV using data recorded by the ATLAS experiment at the Large Hadron Collider is presented. In a data sample corresponding to an integrated luminosity of 4.6 fb-1 collected in 2011, events are selected that are consistent either with two Z bosons decaying to electrons or muons or with one Z boson decaying to electrons or muons and a second Z boson decaying to neutrinos. The ZZ*->llll and ZZ->llnunu cross sections are measured in restricted phase-space regions. These results are then used to derive the total cross section for ZZ events produced with both Z bosons in the mass range 66 to 116 GeV, sigmaZZtot = 6.7 +-0.7 +0.4-0.3 +-0.3 pb, which is consistent with the Standard Model prediction of 5.89+0.22-0.18 pb calculated at next-to-leading order in QCD. The normalized differential cross sections in bins of various kinematic variables are presented. Finally, the differential event yield as a function of the transverse momentum of the leading Z boson is used to set limits on anomalous neutral triple gauge boson couplings in ZZ production.

==> SignalSystematics.tex <==
Group here all the systematics on the Czz, Azz and the estimated number of SM signal events.



==> ZZBib.tex <==
\begin{thebibliography}{99}

\bibitem{Campbell:2011}
  J.~M.~Campbell, R.~K.~Ellis and C.~Williams,
  %``Vector boson pair production at the LHC,''
  JHEP {\bf 1107}, 018 (2011)
  [arXiv:1105.0020 [hep-ph]].
  %%CITATION = JHEPA,1107,018;%%

\bibitem{Gounaris:2000dn}
  G.~J.~Gounaris, J.~Layssac and F.~M.~Renard,
  %``Off-shell structure of the anomalous $Z$ and $\gamma$ selfcouplings,''
  Phys.\ Rev.\  D {\bf 62}, 073012 (2000)
  [arXiv:hep-ph/0005269].
  %%CITATION = PHRVA,D62,073012;%%

\bibitem{Ellison:1998}
  J.~Ellison and J.~Wudka,
  %``Study of trilinear gauge boson couplings at the Tevatron collider,''
  Ann.\ Rev.\ Nucl.\ Part.\ Sci.\  {\bf 48}, 33 (1998)
  [arXiv:hep-ph/9804322].
  %%CITATION = ARNUA,48,33;%%

\bibitem{Acciarri:1999ug}
  M.~Acciarri {\it et al.}  [L3 Collaboration],
  %``Study of $Z$ Boson Pair Production in $e^{+} e^{-}$ collisions at LEP at
  %$S^{(1/2)}$ = 189-GeV,''
  Phys.\ Lett.\  B {\bf 465}, 363 (1999)
  [arXiv:hep-ex/9909043].
  %%CITATION = PHLTA,B465,363;%%

\bibitem{Baur:2000ae}
  U.~Baur and D.~L.~Rainwater,
  %``Probing neutral gauge boson selfinteractions in $Z Z$ production at hadron
  %colliders,''
  Phys.\ Rev.\  D {\bf 62}, 113011 (2000)
  [arXiv:hep-ph/0008063].
  %%CITATION = PHRVA,D62,113011;%%

B
B

\bibitem{Barate:1999jj}
  R.~Barate {\it et al.}  [ALEPH Collaboration],
  %``Measurement of the e+ e- ---> Z Z production cross-section at
  %center-of-mass energies of 183-GeV and 189-GeV,''
  Phys.\ Lett.\  B {\bf 469}, 287 (1999)
  [arXiv:hep-ex/9911003].
  %%CITATION = PHLTA,B469,287;%%


\bibitem{Abdallah:2003dv}
  J.~Abdallah {\it et al.}  [DELPHI Collaboration],
  %``ZZ production in e+ e- interactions at s**(1/2) = 183-GeV to 209-GeV,''
  Eur.\ Phys.\ J.\  C {\bf 30}, 447 (2003)
  [arXiv:hep-ex/0307050].
  %%CITATION = EPHJA,C30,447;%%

\bibitem{Abbiendi:2003va}
  G.~Abbiendi {\it et al.}  [OPAL Collaboration],
  %``Study of Z pair production and anomalous couplings in e+ e- collisions at
  %s**(1/2) between 190-GeV and 209-GeV,''
  Eur.\ Phys.\ J.\  C {\bf 32}, 303 (2003)
  [arXiv:hep-ex/0310013].
  %%CITATION = EPHJA,C32,303;%%

\bibitem{bib:LEPEW2006}
  J.~Alcaraz {\it et al.}  [ALEPH Collaboration and DELPHI Collaboration and
                  L3 Collaboration and ],
  %``A Combination of preliminary electroweak measurements and constraints on
  %the standard model,''
  arXiv:hep-ex/0612034.
  %%CITATION = HEP-EX/0612034;%%

\bibitem{bib:D0_ZZ1}
  V.~M.~Abazov {\it et al.}  [D0 Collaboration],
  %``Search for $ZZ$ and $Z\gamma^*$ production in $p\bar{p}$ collisions at
  %$\sqrt{s}$ = 1.96 TeV and limits on anomalous $ZZZ$ and $ZZ\gamma^*$
  %couplings,''
  Phys.\ Rev.\ Lett.\  {\bf 100}, 131801 (2008)
  [arXiv:0712.0599 [hep-ex]].
  %%CITATION = PRLTA,100,131801;%%

\bibitem{bib:D0_ZZ2}
  V.~M.~Abazov {\it et al.}  [D0 Collaboration],
  %``Observation of $Z Z$ production in $p \bar{p}$ collisions at $\sqrt{s}$ =
  %1.96-TeV,''
  Phys.\ Rev.\ Lett.\  {\bf 101}, 171803 (2008)
  [arXiv:0808.0703 [hep-ex]].
  %%CITATION = PRLTA,101,171803;%%

\bibitem{bib:D0_ZZ3}
  V.~M.~Abazov {\it et al.}  [D0 Collaboration],
  %``Measurement of the $ZZ$ production cross section in $p\bar{p}$ collisions
  %at $\sqrt{s}=1.96$ TeV,''
  arXiv:1104.3078 [hep-ex].
  %%CITATION = ARXIV:1104.3078;%%

\bibitem{bib:CDF_ZZ}
  T.~Aaltonen {\it et al.}  [CDF Collaboration],
  %``First Measurement of $Z Z$ Production in panti-p Collisions at $\sqrt{s}$ =
  %1.96-TeV,''
  Phys.\ Rev.\ Lett.\  {\bf 100}, 201801 (2008)
  [arXiv:0801.4806 [hep-ex]].
  %%CITATION = PRLTA,100,201801;%%

\bibitem{ATLAS-lumi2011}
  [ATLAS collaboration],
  Note in preparation
  
\bibitem{pythia}
  T.~Sjostrand, P.~Eden, C.~Friberg, L.~Lonnblad, G.~Miu, S.~Mrenna and E.~Norrbin,
  %``High-energy physics event generation with PYTHIA 6.1,''
  Comput.\ Phys.\ Commun.\  {\bf 135}, 238 (2001)
  [arXiv:hep-ph/0010017].
  %%CITATION = CPHCB,135,238;%%


\bibitem{bib:MRST2007LOmod}
  A.~Sherstnev and R.~S.~Thorne,
  %``Parton Distributions for LO Generators,''
  Eur.\ Phys.\ J.\  C {\bf 55}, 553 (2008)
  [arXiv:0711.2473 [hep-ph]].
  %%CITATION = EPHJA,C55,553;%%

\bibitem{bib:ATLASDetectorPaper}
  G.~Aad {\it et al.}  [ATLAS Collaboration],
  %``The ATLAS Experiment at the CERN Large Hadron Collider,''
  JINST {\bf 3}, S08003 (2008).
  %%CITATION = JINST,3,S08003;%%

\bibitem{bib:ATLASMCPaper}
  G.~Aad {\it et al.}  [ATLAS Collaboration],
  %``The ATLAS Simulation Infrastructure,''
  Eur.\ Phys.\ J.\  C {\bf 70}, 823 (2010)
  [arXiv:1005.4568 [physics.ins-det]].
  %%CITATION = EPHJA,C70,823;%%


\bibitem{bib:geant4a}
  S.~Agostinelli {\it et al.}  [GEANT4 Collaboration],
  %``GEANT4: A Simulation toolkit,''
  Nucl.\ Instrum.\ Meth.\  A {\bf 506}, 250 (2003).
  %%CITATION = NUIMA,A506,250;%%


\bibitem{bib:MSTW2008}
  A.~D.~Martin, W.~J.~Stirling, R.~S.~Thorne and G.~Watt,
  %``Parton distributions for the LHC,''
  Eur.\ Phys.\ J.\  C {\bf 63}, 189 (2009)
  [arXiv:0901.0002 [hep-ph]].
  %%CITATION = EPHJA,C63,189;%%


\bibitem{Gleisberg:2008ta}
  T.~Gleisberg, S.~Hoeche, F.~Krauss, M.~Schonherr, S.~Schumann, F.~Siegert and J.~Winter,
  %``Event generation with SHERPA 1.1,''
  JHEP {\bf 0902}, 007 (2009)
  [arXiv:0811.4622 [hep-ph]].
  %%CITATION = JHEPA,0902,007;%%

\bibitem{Bella:2008wc}
  G.~Bella,
  %``Weighting Di-Boson Monte Carlo Events in Hadron Colliders,''
  arXiv:0803.3307 [hep-ph].
  %%CITATION = ARXIV:0803.3307;%%

\bibitem{ATLAS-CONF-2011-063}
  ATLAS Collaboration,
  ATLAS-CONF-2011-063.

\end{thebibliography}

